Multigrid Neural Memory

We introduce a novel approach to endowing neural networks with emergent, long-term, large-scale memory. Distinct from strategies that connect neural networks to external memory banks via intricately crafted controllers and hand-designed attentional mechanisms, our memory is internal, distributed, co-located alongside computation, and implicitly addressed, while being drastically simpler than prior efforts. Architecting networks with multigrid structure and connectivity, while distributing memory cells alongside computation throughout this topology, we observe the emergence of coherent memory subsystems. Our hierarchical spatial organization, parameterized convolutionally, permits efficient instantiation of large-capacity memories, while multigrid topology provides short internal routing pathways, allowing convolutional networks to efficiently approximate the behavior of fully connected networks. Such networks have an implicit capacity for internal attention; augmented with memory, they learn to read and write specific memory locations in a dynamic data-dependent manner. We demonstrate these capabilities on exploration and mapping tasks, where our network is able to self-organize and retain long-term memory for trajectories of thousands of time steps. On tasks decoupled from any notion of spatial geometry: sorting, associative recall, and question answering, our design functions as a truly generic memory and yields excellent results.

==> Makefile <==
# programs
PDFLATEX = pdflatex
CP       = cp
RM       = rm
GREP     = grep
DIFF     = diff -q
TOUCH    = touch

# input and output files
TEXFILE = nmg-mem_arxiv.tex
PDFFILE = nmg-mem_arxiv.pdf
TEXINCLUDES = $(wildcard include/*)

# intermediate files
TEXLOG     = $(basename $(TEXFILE)).log
AUXFILE    = $(basename $(TEXFILE)).aux
OUTFILE    = $(basename $(TEXFILE)).out
OLDAUXFILE = $(AUXFILE).old

# arxiv submission files
ARXIV_FILES := $(if $(wildcard files.txt),$(shell cat files.txt),)
ARXIV_OUT   := arxiv.tar.gz

# If this message appears in TEXLOG, we must re-run LaTeX.
RERUNLATEX = "Rerun to get cross-references right"

# The primary target (created by the command "make") is the PDF file.
.PHONY: pdf
pdf: $(PDFFILE)

# This rule uses PDFLaTeX to create a PDF file from a LaTeX file.
# Then PDFLaTeX is re-run to resolve references, as necessary.
$(PDFFILE): $(TEXFILE) $(TEXINCLUDES)
	$(TOUCH) $(AUXFILE)
	$(CP) $(AUXFILE) $(OLDAUXFILE)
	$(PDFLATEX) $<
	while $(GREP) -q $(RERUNLATEX) $(TEXLOG); do $(PDFLATEX) $<; done

# arxiv submission
.PHONY: submit
submit: $(ARXIV_OUT)
$(ARXIV_OUT): files.txt $(ARXIV_FILES)
	@COPYFILE_DISABLE=1 tar cvzfh $(ARXIV_OUT) $(ARXIV_FILES)

# This rule cleans out the files made by the make process.
.PHONY: clean
clean:
	$(RM) -f $(AUXFILE)\
                 $(OLDAUXFILE)\
                 $(OUTFILE)\
                 $(TEXLOG)\
                 $(PDFFILE)\
                 $(ARXIV_OUT)

